Phenomenology and cosmology of millicharged particles and experimental prospects for their search

Mirror world, a parallel hidden sector with microphysics identical to ordinary particle physics, can have several interesting phenomenological and astrophysical implications and mirror matter can be a natural candidate for dark matter in the universe. In this thesis we analyze in detail some of its implications in cosmology, in particular at the primordial nucleosynthesis epoch. Big Bang Nucleosynthesis limits require that the temperature T' of the mirror world should be at least twice lower than that of the ordinary world T. We present numerical calculations regarding the nucleosynthesis epoch and calculate the light and heavier element abundances in both ordinary and mirror worlds as a function of x=T'/T. While the mirror world should be essentially Helium dominated, we show that the heavier elements primordial abundances in mirror world can be significantly higher than in the ordinary world. We also study the cosmological bounds on the kinetic mixing between the photon and mirror photon which in fact renders the mirror particles "millicharged" with respect to the ordinary photon, with small electric charges proportional to the photon kinetic mixing parameter. These bounds are important regarding the possibility of mirror dark matter detection in the DAMA/Libra experiment. This Diploma Thesis was defended in the University of L'Aquila in October 2007.

==> files/Intro.tex <==
\section{Used symbols}
%
$e$ = electron; e.g. $\rho_{el}$ stands for electron energy density.\\
$e^{\pm}$ = electron/positron; e.g. $\rho_{el}$ stands for electron/positron energy density.\\
%
%
\subsection{The greek ones} 
%
$\gamma$ = neutrino; e.g. $\rho_{\gamma}$ stands for electron energy density.\\
$\nu$ = neutrino; e.g. $\rho_{\nu}$ stands for electron energy density.\\

\newpage
